Beyond Subspace Isolation: Many-to-Many Transformer for Light Field Image Super-resolution

The effective extraction of spatial-angular features plays a crucial role in light field image super-resolution (LFSR) tasks, and the introduction of convolution and Transformers leads to significant improvement in this area. Nevertheless, due to the large 4D data volume of light field images, many existing methods opted to decompose the data into a number of lower-dimensional subspaces and perform Transformers in each sub-space individually. As a side effect, these methods inadvertently restrict the self-attention mechanisms to a One-to-One scheme accessing only a limited subset of LF data, explicitly preventing comprehensive optimization on all spatial and angular cues. In this paper, we identify this limitation as subspace isolation and introduce a novel Many-to-Many Transformer (M2MT) to address it. M2MT aggregates angular information in the spatial subspace before performing the self-attention mechanism. It enables complete access to all information across all sub-aperture images (SAIs) in a light field image. Consequently, M2MT is enabled to comprehensively capture long-range correlation dependencies. With M2MT as the foundational component, we develop a simple yet effective M2MT network for LFSR. Our experimental results demonstrate that M2MT achieves state-of-the-art performance across various public datasets, and it offers a favorable balance between model performance and efficiency, yielding higher-quality LFSR results with substantially lower demand for memory and computation. We further conduct in-depth analysis using local attribution maps (LAM) to obtain visual interpretability, and the results validate that M2MT is empowered with a truly non-local context in both spatial and angular subspaces to mitigate subspace isolation and acquire effective spatial-angular representation.

==> tex/tables/AblationStudyNumberCB.tex <==
\begin{table}[t!]
    \centering
    \caption{Ablation study on varing the number of correlation blocks. The best PSNR/SSIM are in bold.}
    \label{tab:ablation_number_blocks}
    \resizebox{.45\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline

    Number    & 6       & 7         & 8                 & 9         & 10        \\ \hline
    PSNR      & 29.60   & 29.69     & \textbf{29.80}    & 29.65     & 29.66     \\
    SSIM      & 0.9257  & 0.9270    & \textbf{0.9277}   & 0.9270    & 0.9271    \\
    \hline
    
    \end{tabular}
    }
\end{table}
